Plasmonic metamaterial based virus detection system: a review

Our atmosphere is constantly changing and new pathogens are erupting now and then and the existing pathogens are mutating continuously. Some of these pathogens, such as SARS-CoV-2, become so deadly that they put the whole technological advancement of healthcare under challenge. Within this very decade several other deadly virus outbreaks were witnessed by humans such as Zika virus, Ebola virus, MERS-coronavirus etc. Though conventional techniques have succeeded in detecting these viruses to some extent, these techniques are time-consuming, costly, and require trained human-resources. Plasmonic metamaterial-based biosensors might pave the way to low-cost rapid virus detection. So this review discusses in details the latest development in plasmonics and metamaterial-based biosensors for virus, viral particles and antigen detection and the future direction of research in this field. Emergence of quantum properties in biosensing, application of machine learning, artificial intelligence and novel materials in biosensing is also discussed in brief.

==> doc/backup.tex <==
\bio{figs/pic1}
Author biography with author photo.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
\endbio

\bio{figs/pic1}
Author biography with author photo.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
\endbio

\bio{figs/sajid.png}
Dr. Sajid Choudhury is working as an Assistant Professor in the Department of EEE, BUET. Dr. Choudhury completed his PhD from the School of Electrical and Computer Engineering in Purdue University. Dr. Choudhury had the privilege of acquiring skills of both experimental and numerical approaches to solve problems related to photonics. His goal is to establish an independent research career in Bangladesh with multidisciplinary collaborations to attack problems related to food safety, energy, healthcare and communications.
\endbio
